Dispersion for Data-Driven Algorithm Design, Online Learning, and Private Optimization

Data-driven algorithm design, that is, choosing the best algorithm for a specific application, is a crucial problem in modern data science. Practitioners often optimize over a parameterized algorithm family, tuning parameters based on problems from their domain. These procedures have historically come with no guarantees, though a recent line of work studies algorithm selection from a theoretical perspective. We advance the foundations of this field in several directions: we analyze online algorithm selection, where problems arrive one-by-one and the goal is to minimize regret, and private algorithm selection, where the goal is to find good parameters over a set of problems without revealing sensitive information contained therein. We study important algorithm families, including SDP-rounding schemes for problems formulated as integer quadratic programs, and greedy techniques for canonical subset selection problems. In these cases, the algorithm's performance is a volatile and piecewise Lipschitz function of its parameters, since tweaking the parameters can completely change the algorithm's behavior. We give a sufficient and general condition, dispersion, defining a family of piecewise Lipschitz functions that can be optimized online and privately, which includes the functions measuring the performance of the algorithms we study. Intuitively, a set of piecewise Lipschitz functions is dispersed if no small region contains many of the functions' discontinuities. We present general techniques for online and private optimization of the sum of dispersed piecewise Lipschitz functions. We improve over the best-known regret bounds for a variety of problems, prove regret bounds for problems not previously studied, and give matching lower bounds. We also give matching upper and lower bounds on the utility loss due to privacy. Moreover, we uncover dispersion in auction design and pricing problems.

==> overview.tex <==
We introduce a general framework for differentially
private and online optimization, motivated by problems in algorithm design
and computational economics. Problems in these domains are notoriously non-convex and discontinuous. For
example, greedy algorithms typically build a solution by iteratively adding
elements that maximize a scoring rule. Prior work has proposed parameterizing
these scoring rules and tuning the parameter to obtain the best performance for
a given application~\citep{Gupta17:PAC}. Tweaking the scoring rule can
cause a cascade of changes in the algorithm's behavior, so its
performance is discontinuous in its parameters. Similarly, in auction
design, a reserve price slightly below the highest bid nearly maximizes revenue,
while a price slightly above the highest bid generates no revenue. In both of
these settings, utility is a volatile, non-convex function.

There is a flourishing and well-developed literature on online convex
optimization~\citep{NicoloGabor06:PLG,Bubeck15:convex}, but less is known for the
non-convex setting. \citet{Kleinberg2008:MetricBandits} study bandit problems over arbitrary metric spaces with Lipschitz
payout functions, whereas the functions we study are not globally
Lipschitz. \citet{Cohen-Addad17:Online} consider a special case of our
online setting, but limited to piecewise constant, one-dimensional functions.
Meanwhile, literature on private continuous optimization has
focused on convex objectives~\citep{Chaudhuri11:Differentially, Bassily14:ERM}
or applying private optimization procedures to non-convex
objectives~\citep{Abadi2016:DLDP} but without utility guarantees. These techniques do not apply to our setting, where we aim to optimize
piecewise Lipschitz functions.

We present general techniques for online and private optimization
of piecewise Lipschitz functions. We provide a sufficient condition, \emph{dispersion},
defining a broadly applicable family of optimization problems that can be solved
online and privately. Roughly
speaking, a set of piecewise Lipschitz functions is disperse if no small
region contains many discontinuities. Algorithm configuration and computational economics problems with considerable real-world impact reduce to optimizing disperse piecewise Lipschitz functions. Further, we expect that
our dispersion condition is applicable beyond private and online optimization,
opening up an exciting research direction.
Finally, this work answers several open questions: \citet{Cohen-Addad17:Online}
asked how to optimize piecewise Lipschitz functions and \citet{Gupta17:PAC}
asked which algorithm configuration problems can be solved online with no regret
algorithms.


==> prelim.tex <==
We use $\Pi$ to denote an abstract input space. We often refer to an abstract
utility function $u: \Pi \times \configs \to [0,H]$ which maps an element $x \in
\Pi$ and a parameter vector $\vec{\rho}$ in the parameter space $\configs
\subset \R^d$ to a score $u(x,\vec{\rho})$. For all $\rho \in \configs$, we
assume $u(x,\vec{\rho})$ is in some bounded range $[0,H]$. Given a sample
$\sample = \left\{x_1, \dots, x_N\right\}$ of problem instances, we define
average utility to be $U(\sample, \vec{\rho}) = \frac{1}{N}\sum_{i = 1}^N u(x_i,
\vec{\rho})$.

Finally, we define piecewise $L$-Lipschitz functions. Let $f: \configs \to \R$
be a function where $\configs \subseteq \R^d$. Suppose there is a partition of
$\configs$ such that in any one region $R$, $f:R \to \R$ is $L$-Lipschitz. Then
$f$ is a \emph{piecewise $L$-Lipschitz function.} Suppose that $u : \Pi \times
\configs \to [0,H]$ is a function such that $u(x, \cdot)$ is piecewise
$L$-Lipschitz for every $x \in \Pi$.


==> prelim2.tex <==
\noindent\textbf{Problem Setup and Notation.} We
study the problem of maximizing sums of bounded piecewise $L$-Lipschitz
functions. Each function in this sum has the form $u(x_t,
\vec{\rho})$, where $u$ is a utility function measuring the quality of a
parameter vector $\vec{\rho}$ for a problem instance $x_t$. For example, if
$x_t$ is a set of bids and $\vec{\rho}$ is a set of reserve prices, then $u(x_t,
\vec{\rho})$ could be the revenue of the second price auction with those reserves.  We use $\Pi$ to denote an instance space and
$\configs \subset \reals^d$ to denote the $d$-dimensional
parameter space. There is a utility function $u : \Pi \times \configs \to [0,H]$
that maps a problem instance $x \in \Pi$ and a parameter $\vec{\rho} \in
\configs$ to the utility of $\vec{\rho}$ for $x$. We
assume that for each instance $x \in \Pi$, we can partition $\configs$ into sets $\configs_1,
\dots, \configs_K$ such that $u(x,\cdot)$ is Lipschitz on each piece.
We let $B(x,r) = \setc{x' \in \reals^d}{\norm{x-x'} \leq r}$
denote the Euclidean ball of radius $r$ centered at $x$.
